Spot the Difference: A Novel Task for Embodied Agents in Changing Environments

Embodied AI is a recent research area that aims at creating intelligent agents that can move and operate inside an environment. Existing approaches in this field demand the agents to act in completely new and unexplored scenes. However, this setting is far from realistic use cases that instead require executing multiple tasks in the same environment. Even if the environment changes over time, the agent could still count on its global knowledge about the scene while trying to adapt its internal representation to the current state of the environment. To make a step towards this setting, we propose Spot the Difference: a novel task for Embodied AI where the agent has access to an outdated map of the environment and needs to recover the correct layout in a fixed time budget. To this end, we collect a new dataset of occupancy maps starting from existing datasets of 3D spaces and generating a number of possible layouts for a single environment. This dataset can be employed in the popular Habitat simulator and is fully compliant with existing methods that employ reconstructed occupancy maps during navigation. Furthermore, we propose an exploration policy that can take advantage of previous knowledge of the environment and identify changes in the scene faster and more effectively than existing agents. Experimental results show that the proposed architecture outperforms existing state-of-the-art models for exploration on this new setting.

==> sections/dataset.tex <==
\section{Dataset}
In this section, we describe the procedure that we employ to obtain an occupancy maps for an available 3D environment. We then show that, given this map and some semantic knowledge about the scene, it is possible to generate multiple maps representing the same environment in different states.

\subsection{Semantic and Occupancy Map}
Given a 3D environment, we place the agent in a free (navigable) location $(x, y, z)$ with heading $\theta=0$ (facing eastward). We assume that the input consists of a depth image, which could be obtained with a specific sensor or estimated, and a semantic image. The semantic information could be manually annotated (as in our case) or may be obtained using a state-of-the-art semantic segmentation architecture, starting from the RGB image.
If the camera pose and intrinsics are known, than we can project each semantic pixel belonging to the input image into a 2-dimensional top-down semantic map. We perform the same operation after rotating the agent by $\Delta_\theta=15°$, until we perform a complete $360°$ rotation. To cover the full scene, we repeat this procedure placing the agent in each vertex of a grid-like structure, at a distance of $0.5m$ from the previous capture point. The elevation $z$ is instead fixed. During this step, we average the results of subsequent observations of overlapping portions of space.
After the acquisition, we obtain an occupancy map with $C$-channels, where each pixel corresponds to a $5cm^2$ portion of space in the real environment. For each semantic channel $c \in [0, C)$, pixel values represent the probability that the corresponding portion of space in the 3D environment is occupied by an object of semantic class $c$.

\subsection{Alternative States for the Environments}
The semantic maps obtained in the previous step represent one possible state for the corresponding 3D environments. However, if even a small element in the scene were to be moved in a slightly different position, then we expect to observe a similar change in the semantic map. We could say that we would see the same environment in a different state. For photorealistic environments, it is unfeasible to capture multiple 3D scans at different times to achieve such diversity, mainly because of the high costs in terms of time and resources needed for a 3D acquisition from the real-world. Instead of manipulating the real-world scene (changing the furniture position, removing chairs, etc.), we propose to perform a combination of two simple operations on the acquired semantic maps: \textbf{deletion} and \textbf{displacement}. By doing so, we can simulate displacements or removals of real objects in the scene. For each semantic channel, we isolate the single elements belonging to that particular semantic category using an algorithm for connected component labeling. Then, we sample a subset of elements to delete from the scene, and a subset of items that must be re-positioned in a new and free location of the map. During this phase, we consider categories that have a high probability of being displaced or removed in the real world, while we ignore non-movable semantic categories such as \textit{fireplaces}, \textit{columns}, and \textit{stairs}. After this step, we obtain a map representing a possible state for the environment, which could be very different from the one in which the 3D acquisition was taken.

\subsection{Dataset Details}
To create our dataset, we start from the Matterport 3D dataset of spaces~\cite{chang2017matterport3d}, which comprises 90 different building scans and is enriched with dense semantic annotations. Then, we consider each floor in the building and we compute the occupancy semantic map for that floor. For each map, we then create 10 alternative versions of that same environment using the algorithm described above. In this step, we discard floors that have few semantic objects (\eg~empty rooftops) or that are not fully navigable by the agent. In total, we keep 249 floors belonging to 81 different buildings, thus generating a total of 2490 different states for these floors. We then divide the dataset in three different splits: train (58 spaces and 207 floors), validation (9 spaces and 16 floors), and test (14 spaces and 26 floors).
We repeat the same process with a subset of GibsonEnv, enriched with semantic annotations from (cite). In this case we create a total of 680 possible maps from 30 different spaces. We separate the data in a training set with 25 spaces and 55 floors; and a validation set consisting of 5 spaces and 13 floors.
